BEVContrast: Self-Supervision in BEV Space for Automotive Lidar Point Clouds

We present a surprisingly simple and efficient method for self-supervision of 3D backbone on automotive Lidar point clouds. We design a contrastive loss between features of Lidar scans captured in the same scene. Several such approaches have been proposed in the literature from PointConstrast, which uses a contrast at the level of points, to the state-of-the-art TARL, which uses a contrast at the level of segments, roughly corresponding to objects. While the former enjoys a great simplicity of implementation, it is surpassed by the latter, which however requires a costly pre-processing. In BEVContrast, we define our contrast at the level of 2D cells in the Bird's Eye View plane. Resulting cell-level representations offer a good trade-off between the point-level representations exploited in PointContrast and segment-level representations exploited in TARL: we retain the simplicity of PointContrast (cell representations are cheap to compute) while surpassing the performance of TARL in downstream semantic segmentation.

==> tables/transfer.tex <==
\begin{table*}
% \small
\setlength{\tabcolsep}{8pt}
\centering

\begin{tabular}{@{}ll|cc|cc|cc|cc|cc@{}}

\toprule
Dataset & Method & \multicolumn{2}{c}{0.1\%} & \multicolumn{2}{c}{1\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c}{50\%} & \multicolumn{2}{c}{100\%}\\

% SemanticKITTI to SemanticPOSS
\midrule%\midrule
\multirow{8}{*}{SK $\rightarrow$ SP} & No pre-training & 36.9 & \std{0.5} & 46.4 & \std{0.3} & 54.5 & \std{0.4} & 55.3 & \std{0.2} &  55.1 & \std{0.4} \\
& PointContrast\ddag~\cite{pointcontrast} & 39.3 & \std{0.8} & 48.1 & \std{0.6} & 55.1 & \std{0.5} & 56.2 & \std{0.6} & 56.2 & \std{0.6} \\
& SegContrast~\cite{segcontrast} & 41.7 & \std{0.8} & 49.4 & \std{0.4} & 55.4 & \std{0.2} & 56.2 & \std{0.9} & 56.4 & \std{0.5} \\
& DepthContrast\dag~\cite{depthcontrast} & 39.7 & \std{0.9} & 48.5 & \std{0.4} & \rtwo{55.8} & \std{0.4} & 56.0 & \std{0.8} & 56.5 & \std{0.5} \\
& STSSL~\cite{stssl} & 40.2 & \std{0.5} & 49.2 & \std{0.5} & 55.5 & \std{0.4} & \rone{56.8} & \std{0.8} & 56.2 & \std{1.0} \\
& ALSO~\cite{also} & 40.7 & \std{0.7} & 49.6 & \std{0.7} & \rtwo{55.8} & \std{0.5} & 56.4 & \std{0.6} & \rtwo{56.7} & \std{1.1} \\
& TARL~\cite{TARL} & \rone{45.8} & \std{0.6} & \rone{52.2} & \std{0.5} & \rone{56.0} & \std{0.3} & \rone{56.8} & \std{0.4} & \rone{57.0} & \std{0.6} \\
& \textit{\ours (ours)} & \rtwo{42.9} & \std{0.5} & \rtwo{51.9} & \std{0.7} & 55.7 & \std{0.4} & \rtwo{56.7} & \std{0.5} & 56.4 & \std{0.3} \\


\bottomrule
\\[-3.5mm]
\multicolumn{12}{c}{\dag\,as reimplemented by ALSO~\cite{also} \hspace{35pt} \ddag\,as reimplemented by SegContrast~\cite{segcontrast}}
\\
\end{tabular}
\vspace*{-3mm}
\caption{
\textbf{Semantic segmentation fine-tuning results on SemanticPOSS} after pretraining on SemanticKITTI. Different subsets from $0.1\%$ to $100\%$ of the training set of SemanticPOSS are used for fine-tuning. We report the average and standard deviation of the mIoU\% over 5 different fine-tuning. The individual fine-tuning results are in the supplementary material.
}
\label{table:transfer}
    
\end{table*}
